Applying and Extending the Delta Debugging Algorithm for Elevator Dispatching Algorithms (Experience Paper)

Elevator systems are one kind of Cyber-Physical Systems (CPSs), and as such, test cases are usually complex and long in time. This is mainly because realistic test scenarios are employed (e.g., for testing elevator dispatching algorithms, typically a full day of passengers traveling through a system of elevators is used). However, in such a context, when needing to reproduce a failure, it is of high benefit to provide the minimal test input to the software developers. This way, analyzing and trying to localize the root-cause of the failure is easier and more agile. Delta debugging has been found to be an efficient technique to reduce failure-inducing test inputs. In this paper, we enhance this technique by first monitoring the environment at which the CPS operates as well as its physical states. With the monitored information, we search for stable states of the CPS during the execution of the simulation. In a second step, we use such identified stable states to help the delta debugging algorithm isolate the failure-inducing test inputs more efficiently. We report our experience of applying our approach into an industrial elevator dispatching algorithm. An empirical evaluation carried out with real operational data from a real installation of elevators suggests that the proposed environment-wise delta debugging algorithm is between 1.3 to 1.8 times faster than the traditional delta debugging, while producing a larger reduction in the failure-inducing test inputs. The results provided by the different implemented delta debugging algorithm versions are qualitatively assessed with domain experts. This assessment provides new insights and lessons learned, such as, potential applications of the delta debugging algorithm beyond debugging.

==> Tables/RQ1Table.tex <==
\begin{table*}[ht]
\centering
\caption{(RQ1) Summary of the performed statistical test for the Execution Time metric}
\label{table:RQ1}
\begin{tabular}{lllllllll}
\cline{4-9}
\textbf{}             & \textbf{}                 & \textbf{}            & \multicolumn{2}{c}{\textbf{Test 1}} & \multicolumn{2}{c}{\textbf{Test 2}} & \multicolumn{2}{c}{\textbf{Test 2}} \\ \hline
\textbf{Threshold \%} & \textbf{Algorithm A}      & \textbf{Algorithm B} & \textbf{A12}   & \textbf{p-value}   & \textbf{A12}   & \textbf{p-value}   & \textbf{A12}   & \textbf{p-value}   \\ \hline
\multirow{4}{*}{5\%}  & \multirow{4}{*}{Backward} & $DD_{TB}$            & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $DD_{EB}$            & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $EWDD_{TB}$          & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $EWDD_{EB}$          & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\ \hline
\multirow{4}{*}{7\%}  & \multirow{4}{*}{Backward} & $DD_{TB}$            & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $DD_{EB}$            & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $EWDD_{TB}$          & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $EWDD_{EB}$          & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\ \hline
\multirow{4}{*}{9\%}  & \multirow{4}{*}{Backward} & $DD_{TB}$            & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $DD_{EB}$            & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $EWDD_{TB}$          & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $EWDD_{EB}$          & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\ \hline
\multirow{4}{*}{10\%} & \multirow{4}{*}{Backward} & $DD_{TB}$            & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $DD_{EB}$            & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $EWDD_{TB}$          & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $EWDD_{EB}$          & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\ \hline
\multirow{4}{*}{11\%} & \multirow{4}{*}{Backward} & $DD_{TB}$            & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $DD_{EB}$            & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $EWDD_{TB}$          & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $EWDD_{EB}$          & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\ \hline
\multirow{4}{*}{13\%} & \multirow{4}{*}{Backward} & $DD_{TB}$            & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $DD_{EB}$            & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $EWDD_{TB}$          & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $EWDD_{EB}$          & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\ \hline
\multirow{4}{*}{15\%} & \multirow{4}{*}{Backward} & $DD_{TB}$            & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $DD_{EB}$            & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $EWDD_{TB}$          & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $EWDD_{EB}$          & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\ \hline
\multirow{4}{*}{17\%} & \multirow{4}{*}{Backward} & $DD_{TB}$            & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $DD_{EB}$            & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $EWDD_{TB}$          & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $EWDD_{EB}$          & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\ \hline
\multirow{4}{*}{19\%} & \multirow{4}{*}{Backward} & $DD_{TB}$            & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $DD_{EB}$            & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $EWDD_{TB}$          & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $EWDD_{EB}$          & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\ \hline
\multirow{4}{*}{20\%} & \multirow{4}{*}{Backward} & $DD_{TB}$            & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $DD_{EB}$            & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $EWDD_{TB}$          & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\
                      &                           & $EWDD_{EB}$          & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  & 1              & \textless{}0.0001  \\ \hline
\end{tabular}
\end{table*}



==> Tables/RQ2Table.tex <==
\begin{table*}[ht]
\centering
\caption{RQ2 -- Summary of the statistical test results for the Execution Time metric}
\label{table:RQ2}
\begin{tabular}{lllllllll}
\cline{4-9}
                                          &                                          &                                          & \multicolumn{2}{c}{\textbf{Test input 1}} & \multicolumn{2}{c}{\textbf{Test input 2}} & \multicolumn{2}{c}{\textbf{Test input 3}} \\ \hline
\multicolumn{1}{c}{\textbf{Threshold \%}} & \multicolumn{1}{c}{\textbf{Algorithm A}} & \multicolumn{1}{c}{\textbf{Algorithm B}} & \textbf{\^{A}$_{12}$}   & \textbf{p-value}   & \textbf{\^{A}$_{12}$}   & \textbf{p-value}   & \textbf{\^{A}$_{12}$}   & \textbf{p-value}   \\ \hline
\multirow{2}{*}{5\%}                      & DD\textsubscript{TB}                                   & EWDD\textsubscript{TB}                                 & 1.00             & \textless{}0.0001  & 1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  \\
                                          & DD\textsubscript{EB}                              & EWDD\textsubscript{EB}                            &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  \\ \hline
\multirow{2}{*}{7\%}                      & DD\textsubscript{TB}                                   & EWDD\textsubscript{TB}                                 &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  \\
                                          & DD\textsubscript{EB}                              & EWDD\textsubscript{EB}                            &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  \\ \hline
\multirow{2}{*}{9\%}                      & DD\textsubscript{TB}                                   & EWDD\textsubscript{TB}                                 &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  \\
                                          & DD\textsubscript{EB}                              & EWDD\textsubscript{EB}                            &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  \\ \hline
\multirow{2}{*}{10\%}                     & DD\textsubscript{TB}                                   & EWDD\textsubscript{TB}                                 &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  \\
                                          & DD\textsubscript{EB}                              & EWDD\textsubscript{EB}                            &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  \\ \hline
\multirow{2}{*}{11\%}                     & DD\textsubscript{TB}                                   & EWDD\textsubscript{TB}                                 &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  \\
                                          & DD\textsubscript{EB}                              & EWDD\textsubscript{EB}                            &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  \\ \hline
\multirow{2}{*}{13\%}                     & DD\textsubscript{TB}                                   & EWDD\textsubscript{TB}                                 &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  \\
                                          & DD\textsubscript{EB}                              & EWDD\textsubscript{EB}                            & 0.99         & \textless{}0.0001  &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  \\ \hline
\multirow{2}{*}{15\%}                     & DD\textsubscript{TB}                                   & EWDD\textsubscript{TB}                                 &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  \\
                                          & DD\textsubscript{EB}                              & EWDD\textsubscript{EB}                            &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  \\ \hline
\multirow{2}{*}{17\%}                     & DD\textsubscript{TB}                                   & EWDD\textsubscript{TB}                                 &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  \\
                                          & DD\textsubscript{EB}                              & EWDD\textsubscript{EB}                            &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  \\ \hline
\multirow{2}{*}{19\%}                     & DD\textsubscript{TB}                                   & EWDD\textsubscript{TB}                                 &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  \\
                                          & DD\textsubscript{EB}                              & EWDD\textsubscript{EB}                            &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  \\ \hline
\multirow{2}{*}{20\%}                     & DD\textsubscript{TB}                                   & EWDD\textsubscript{TB}                                 &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  \\
                                          & DD\textsubscript{EB}                              & EWDD\textsubscript{EB}                            & 0.99         & \textless{}0.0001  &1.00             & \textless{}0.0001  &1.00             & \textless{}0.0001  \\ \hline
\end{tabular}

\end{table*}

==> TimeTable.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht]
\centering
\begin{tabular}{lllllllllll}
\cline{3-11}
                      &                    & \multicolumn{3}{c}{\textbf{Test 1}}               & \multicolumn{3}{c}{\textbf{Test 2}}               & \multicolumn{3}{c}{\textbf{Test 3}}               \\ \hline
\textbf{Threshold \%} & \textbf{Algorithm} & \textbf{$m$} & \textbf{$\mu$} & \textbf{$\sigma$} & \textbf{$m$} & \textbf{$\mu$} & \textbf{$\sigma$} & \textbf{$m$} & \textbf{$\mu$} & \textbf{$\sigma$} \\ \hline
\multirow{4}{*}{5\%}  & $DD_{PB}$          & 643.09       & 575.1          & 224.06            & 419.93       & 385.94         & 89.24             & 475.1        & 463.91         & 107.54            \\
                      & $DD_{TB}$          & 559.12       & 527.24         & 107.75            & 426.9        & 388.51         & 79.47             & 423.72       & 376.71         & 119.21            \\
                      & $EWDD_{PB}$        & 375.27       & 367.65         & 29.15             & 290.37       & 290.28         & 11.02             & 280.77       & 281.09         & 11.71             \\
                      & $EWDD_{TB}$        & 300.16       & 303.6          & 19.84             & 269.38       & 267.61         & 10.91             & 238.26       & 241.24         & 7.76              \\ \hline
\multirow{4}{*}{7\%}  & $DD_{PB}$          & 607.66       & 556.22         & 158.56            & 411.78       & 386.77         & 63.99             & 453.48       & 431.45         & 51.19             \\
                      & $DD_{TB}$          & 564.89       & 514.54         & 167.26            & 443.61       & 408.82         & 96.95             & 404.22       & 366.54         & 88.5              \\
                      & $EWDD_{PB}$        & 364.16       & 362.01         & 17.57             & 290.3        & 290.03         & 12.82             & 281.15       & 279.06         & 13.37             \\
                      & $EWDD_{TB}$        & 290.74       & 286.12         & 13.87             & 267.24       & 267.59         & 11.27             & 239.58       & 235.31         & 14.6              \\ \hline
\multirow{4}{*}{9\%}  & $DD_{PB}$          & 588.56       & 558.71         & 115.9             & 399.13       & 390.91         & 42.63             & 457.43       & 445.49         & 57.04             \\
                      & $DD_{TB}$          & 552.35       & 507.21         & 122.3             & 434.48       & 408.69         & 67.17             & 390.52       & 372.36         & 43.26             \\
                      & $EWDD_{PB}$        & 371.18       & 363.41         & 25.78             & 291.18       & 289.36         & 15.34             & 284.28       & 282.22         & 12.5              \\
                      & $EWDD_{TB}$        & 297.69       & 302.39         & 15.74             & 249.79       & 245.1          & 14.47             & 240.41       & 234.81         & 14.16             \\ \hline
\multirow{4}{*}{10\%} & $DD_{PB}$          & 585.17       & 566.03         & 116.01            & 398.46       & 384.87         & 41.8              & 444.58       & 429.69         & 46.09             \\
                      & $DD_{TB}$          & 540.4        & 519.64         & 89.95             & 425.82       & 408.08         & 39.51             & 387.58       & 373.44         & 41.82             \\
                      & $EWDD_{PB}$        & 370.89       & 359.21         & 24.4              & 288.91       & 289.46         & 12.17             & 279.59       & 278.79         & 11.37             \\
                      & $EWDD_{TB}$        & 293.56       & 292.52         & 13.43             & 243.28       & 244.38         & 10.18             & 236.57       & 234.3          & 10.91             \\ \hline
\multirow{4}{*}{11\%} & $DD_{PB}$          & 577.26       & 558.71         & 106.93            & 403.5        & 379.73         & 53.83             & 461.29       & 424.99         & 81.3              \\
                      & $DD_{TB}$          & 535.89       & 512.95         & 87.98             & 423.37       & 402.71         & 45.71             & 389.98       & 373.25         & 44.6              \\
                      & $EWDD_{PB}$        & 364.95       & 358.3          & 19.63             & 291.46       & 292.12         & 13.7              & 284.13       & 284.41         & 14.33             \\
                      & $EWDD_{TB}$        & 293.21       & 297.77         & 11.93             & 247.53       & 245.78         & 13.29             & 238.11       & 235.85         & 10.24             \\ \hline
\multirow{4}{*}{13\%} & $DD_{PB}$          & 537.25       & 505.21         & 118.53            & 426.33       & 393.32         & 102.03            & 475.15       & 448.52         & 95.38             \\
                      & $DD_{TB}$          & 497.92       & 468.53         & 55.54             & 425.23       & 401.55         & 42.1              & 396.41       & 373.55         & 59.01             \\
                      & $EWDD_{PB}$        & 371.6        & 376.1          & 23.53             & 289.46       & 289.6          & 12.01             & 282.5        & 278.91         & 13.58             \\
                      & $EWDD_{TB}$        & 292.93       & 290.94         & 13.43             & 246.25       & 244.71         & 11.53             & 240.98       & 239.59         & 13.96             \\ \hline
\multirow{4}{*}{15\%} & $DD_{PB}$          & 526.32       & 509.22         & 88.37             & 410          & 385.48         & 68.22             & 447.42       & 435.67         & 45.97             \\
                      & $DD_{TB}$          & 505.16       & 480.39         & 50.95             & 428.02       & 401.34         & 45.26             & 394.1        & 375.11         & 53.29             \\
                      & $EWDD_{PB}$        & 367.84       & 361.76         & 22.85             & 290.52       & 289.52         & 12.88             & 281.13       & 279.44         & 13.65             \\
                      & $EWDD_{TB}$        & 299.26       & 304.6          & 16.34             & 248.16       & 245.36         & 14.13             & 237.67       & 235.18         & 10.43             \\ \hline
\multirow{4}{*}{17\%} & $DD_{PB}$          & 517.06       & 512.79         & 65.56             & 396.54       & 369.89         & 47.04             & 446.56       & 432.57         & 46.45             \\
                      & $DD_{TB}$          & 501.36       & 485.43         & 42.74             & 430.08       & 405.95         & 47.19             & 392.47       & 373.4          & 46.81             \\
                      & $EWDD_{PB}$        & 366.92       & 365.46         & 21.04             & 289.85       & 290.18         & 12.33             & 281.34       & 279.28         & 14.12             \\
                      & $EWDD_{TB}$        & 294.59       & 292.3          & 13.45             & 244.51       & 244.64         & 9.89              & 239.85       & 235.07         & 11.21             \\ \hline
\multirow{4}{*}{19\%} & $DD_{PB}$          & 511.95       & 500.71         & 60.82             & 397.06       & 379.82         & 43.5              & 438.18       & 433.07         & 44.21             \\
                      & $DD_{TB}$          & 524.45       & 490.99         & 87.1              & 456.68       & 408.47         & 113.77            & 421.74       & 384.3          & 110.52            \\
                      & $EWDD_{PB}$        & 370.09       & 365.35         & 24.1              & 288.1        & 289.48         & 9.7               & 281.07       & 278.54         & 13.49             \\
                      & $EWDD_{TB}$        & 294.37       & 292.85         & 12.22             & 249.97       & 246.26         & 12.33             & 239.45       & 235.81         & 12.36             \\ \hline
\multirow{4}{*}{20\%} & $DD_{PB}$          & 509.82       & 514.63         & 60.61             & 413.01       & 392.69         & 75.15             & 476.09       & 452.45         & 94.58             \\
                      & $DD_{TB}$          & 525.28       & 483.81         & 111.99            & 439.72       & 407.05         & 66.72             & 403.75       & 381.5          & 60.38             \\
                      & $EWDD_{PB}$        & 367.34       & 354.7          & 25.07             & 291.34       & 289.64         & 14.07             & 283.33       & 279.25         & 16.46             \\
                      & $EWDD_{TB}$        & 298.65       & 303.14         & 14.96             & 246.52       & 244.76         & 12.02             & 240.61       & 239.69         & 11.9              \\ \hline
\end{tabular}
\end{table*}

==> background.tex <==



% CPSs combine digital cyber technologies with paralell physical proceses \pablo{cita}. These systems contain different abstractiosn for physical and computational elements and their interactions. An example of a CPS is the elevator dispatcher, which requieres the integration of physical calculations (to model the state of the elevator) and computations (the control logic). Model-based design is the most commonly used technique to model CPSs, as it allows the integration of the physical elements with the discrete logic that could be translated to software. To this end, MATLAB/Simulink has become the leading  tool\pablo{cite}.

% Compared to software applications, testing CPSs is challenging. On the one hand, verification methods of such systems depend on simulation-based testing. This technique is expensive since complex mathematical models are used to model the physical part of CPSs. For instance, in an industrial case reported in \pablo{cite}, when simulating autonomous vehicles, a simulation run is reduced to 10\% of the real time (e.g., simulating 1 minute takes 10 minutes). 

% On the other hand, CPSs operate in uncertain environments where unexpected scenarios may happen \pablo{cita} (e.g. for an elevator installation it is impossible to predict whether a passenger will arrive or not, so it is impossible to foresee which will be the elevator behavior). It is not possible to verify the system behavior under real conditions until testing is performed on the real hardware, but recent research suggest that most of the bugs can be reproduced and identified in simulation. \pablo{Cite} Nevertheless, simulating such systems is time consuming since the test inputs are long, thus, developers might need to wait long time every time they want to reproduce the failure.

% In order to solve this problem, it has been shown that Delta Debugging Algorithm \pablo{Cita} is effective \pablo{Cita}. This algorithm aims at simplifying the test cases by automatically isolating the difference that causes the failure, so that, the developers will need to wait less time to reproduce the failure. 

 

 
